SceneTex: High-Quality Texture Synthesis for Indoor Scenes via Diffusion Priors

We propose SceneTex, a novel method for effectively generating high-quality and style-consistent textures for indoor scenes using depth-to-image diffusion priors. Unlike previous methods that either iteratively warp 2D views onto a mesh surface or distillate diffusion latent features without accurate geometric and style cues, SceneTex formulates the texture synthesis task as an optimization problem in the RGB space where style and geometry consistency are properly reflected. At its core, SceneTex proposes a multiresolution texture field to implicitly encode the mesh appearance. We optimize the target texture via a score-distillation-based objective function in respective RGB renderings. To further secure the style consistency across views, we introduce a cross-attention decoder to predict the RGB values by cross-attending to the pre-sampled reference locations in each instance. SceneTex enables various and accurate texture synthesis for 3D-FRONT scenes, demonstrating significant improvements in visual quality and prompt fidelity over the prior texture generation methods.

==> figures/scenes.tex <==
\begin{figure*}[!ht]
    \centering
    \includegraphics[width=0.9\linewidth]{assets/scenes.jpg}
    \caption{ 
    Generated textures on 3D-FRONT scenes with different prompts. Image best viewed in color.
    }
    \label{fig:scenes}
\end{figure*}

==> sections/2_related_work_bkup.tex <==
\paragraph{3D generation from 2D and 3D data.}

In the pursuit of 3D generation, it is a logical step to train models directly on 3D data. 
%
In contrast to 2D images, the domain of 3D data offers several distinct representations, each possessing unique characteristics.
%
This diversity has spurred the development of various generative models, including those based on voxels~\cite{lin2023infinicity,siarohin2023unsupervised,smith2017improved,xie2018learning}, point clouds~\cite{achlioptas2018learning,luo2021diffusion}, meshes~\cite{zhang2021sketch2model}, signed distance functions~\cite{chen2019learning,cheng2022sdfusion,cheng2022cross,dai2021spsg,autosdf2022}, and more. 
%
However, unlike the ubiquity of 2D images and videos, 3D data is inherently scarce and poses significant challenges in terms of acquisition and annotation. 
%
As a result, generative models trained on 3D data often produce samples that exhibit limitations in both structural and textural quality and diversity. 
%
Recent efforts have sought to address this issue by utilizing differentiable rendering techniques to learn texture generation from 2D images alone~\cite{gao2022get3d,siddiqui2022texturify, yu2021learning, muller2023diffrf}. 
%
Nevertheless, these models typically demonstrate proficiency in specific shape categories while grappling with the quality of generated textures.
%
Generating 3D shapes on unseen arbitrary categories still remains a challenge task.


\paragraph{Text-to-image generation.}

Recently, significant strides have been made in the field of vision-language integration~\cite{hu2021unit, singh2022flava, wang2022ofa, radford2021learning, chen2022d3net, chen2020scanrefer, chen2021scan2cap, chen2022unit3d}, notably with the introduction of Contrastive Language-Image Pre-Training (CLIP)~\cite{radford2021learning}. 
CLIP's semantically rich representation, honed through training on text-image pairs, has paved the way for text-guided image generation. 
Early efforts~\cite{crowson2022vqgan,patashnik2021styleclip} involved integrating CLIP with various backbones like StyleGAN~\cite{karras2020analyzing} and VQGAN~\cite{esser2021taming}. 
However, there has been a notable shift towards diffusion models~\cite{dhariwal2021diffusion,ho2020denoising,ho2021cascaded,nichol2021improved,saharia2022image}, renowned for their superior visual quality and training stability compared to Generative Adversarial Networks (GANs)~\cite{GANs}, which are now being trained on extensive text-image datasets utilizing CLIP encodings~\cite{kawar2022imagic,ramesh2021zero,Rombach_2022_CVPR}. 
Among these models, Stable Diffusion~\cite{stablediffusion,Rombach_2022_CVPR} has garnered considerable attention, being an open-source framework with numerous extensions~\cite{stablediffusion,zhang2023adding} that support diverse conditional modalities, including text prompts, depth images, poses, sketches, and more. 
Furthermore, the applicability of CLIP has extended into the 3D realm, enabling text-guided generation of 3D shapes and textures~\cite{michel2022text2mesh,mohammad2022clip}. 
In this paper, we take a pre-trained depth-to-image diffusion model as a critic to ensure the consistency of texturing in our framework.

\input{figures/architecture}

\paragraph{Text-guide 3D generation from 2D priors.}

Drawing inspiration from the notable success of Neural Radiance Fields (NeRF)\cite{mildenhall2020nerf}, a family of NeRF-based generators\cite{abdal20233davatargan, EG3D,piGAN, StyleNeRF,Giraffe, or2022stylesdf,GRAF,skorokhodov3d,xu2022discoscene} has emerged, aiming to harness NeRF's capabilities for learning 3D structures from 2D images within GAN-based frameworks. 
This trend has been further enriched by a novel research direction that combines NeRF techniques with the burgeoning domain of diffusion-based text-to-image models, facilitating text-to-3D learning under the constraint of 2D supervision. 
In tackling the optimization challenges inherent in NeRF fields, a score distillation sampling (SDS) loss~\cite{poole2022dreamfusion} has been introduced, leveraging a pretrained 2D diffusion model as a critic to provide crucial gradients. 
Subsequent endeavors have explored the incorporation of this loss within latent spaces~\cite{cheng2022sdfusion,metzer2022latent} and through a coarse-to-fine refinement strategy~\cite{lin2022magic3d}. 
As SDS loss often results in extremely saturated and smooth appearance, follow-up work~\cite{wang2023prolificdreamer} improve SDS through incorporating a variation inference process with a fine-tunable LoRA~\cite{hu2021lora} module.
The variational score distillation sampling (VSD) loss greatly mitigates the over-saturation issue.
Nevertheless, latent space optimization often yields subpar visual quality, primarily due to mismatches between latent features and the target RGB space, as well as the absence of perspective transformations during the decoding of latent codes into RGB pixels. 
Recent work~\cite{richardson2023texture, chen2023text2tex} has proposed a non-optimization approach involving progressive updates from predetermined viewpoints. 
However, autoregressive methods inherent in such approaches face challenges tied to accumulated artifacts and loop closure issues. 
In contrast, our method takes a direct path by optimizing an implicit texture field in high-resolution RGB space, incorporating precise geometric cues, thereby yielding visually captivating and view-consistent high-quality textures.

